An Instance Space Analysis of Constrained Multi-Objective Optimization Problems

Multi-objective optimization problems with constraints (CMOPs) are generally considered more challenging than those without constraints. This in part can be attributed to the creation of infeasible regions generated by the constraint functions, and/or the interaction between constraints and objectives. In this paper, we explore the relationship between constrained multi-objective evolutionary algorithms (CMOEAs) performance and CMOP instances characteristics using Instance Space Analysis (ISA). To do this, we extend recent work focused on the use of Landscape Analysis features to characterise CMOP. Specifically, we scrutinise the multi-objective landscape and introduce new features to describe the multi-objective-violation landscape, formed by the interaction between constraint violation and multi-objective fitness. Detailed evaluation of problem-algorithm footprints spanning six CMOP benchmark suites and fifteen CMOEAs, illustrates that ISA can effectively capture the strength and weakness of the CMOEAs. We conclude that two key characteristics, the isolation of non-dominate set and the correlation between constraints and objectives evolvability, have the greatest impact on algorithm performance. However, the current benchmarks problems do not provide enough diversity to fully reveal the efficacy of CMOEAs evaluated.

==> CMOP - TEVC/Tables/benchmarks.tex <==
\begin{table}[!t]
	\caption{Characteristics of the benchmarks employed in this study. All of them have a scalable number of decision variables. \textit{Type} describes the relationship between $UPF$ and $PF$, $M$ is the number of objectives, $CF$ is the number of constraints, $UPF$ and $PF$ columns define their shape, and the size and connectivity of the feasible region is given in the last column.  \textit{S} is short for scalable, \textit{C} for Controllable, \textit{Disconn} for Disconnected, \textit{Conn} for Connected, \textit{L} for Large, and \textit{S} for Small.}
	\label{tab:bench}
	\scriptsize
	\begin{tabular}{llllllll}
		\toprule
		\textbf{Problem} & \textbf{Type} & \textbf{M} & \textbf{CF} & \textbf{UPF} & \textbf{PF} & \multicolumn{2}{c}{\textbf{Feasible   Region}} \\ \midrule
		CF1              & II            & 2          & 1          & Linear       & Disconn & L/Conn                       \\
		CF2              & II            & 2          & 1          & Convex       & Disconn & L/Conn                       \\
		CF3              & II            & 2          & 1          & Concave      & Disconn & L/Conn                       \\
		CF4              & III           & 2          & 1          & Linear       & Linear       & L/Conn                      \\
		CF5              & III           & 2          & 1          & Linear       & Linear       & L/Conn                      \\
		CF6              & III           & 2          & 1          & Convex       & Mixed        & L/Conn                       \\
		CF7              & III           & 2          & 1          & Convex       & Mixed        & L/Conn                       \\
		CF8              & II            & 3          & 1          & Concave      & Disconn & L/Conn                       \\
		CF9              & II            & 3          & 1          & Concave      & Disconn & L/Conn                       \\
		CF10             & II            & 3          & 1          & Concave      & Disconn & L/Conn                       \\
		C1-DTLZ1         & I             & S          & 1          & Linear       & Linear       & S/Conn                       \\
		C2-DTLZ2         & II            & S          & 1          & Concave      & Concave      & S/Disconn                    \\
		C1-DTLZ3         & I             & S          & 1          & Concave      & Concave      & L/Disconn                    \\
		C3-DTLZ4         & IV            & S          & M          & Concave      & Concave      & L/Conn                       \\
		DC1-DTLZ1        & II            & S          & 1          & Linear       & Disconn & C/Disconn                    \\
		DC1-DTLZ3        & II            & S          & 1          & Concave      & Disconn & C/Disconn                    \\
		DC2-DTLZ1        & I             & S          & 2          & Linear       & Linear       & S/Disconn                    \\
		DC2-DTLZ3        & I             & S          & 2          & Concave      & Concave      & S/Disconn                    \\
		DC3-DTLZ1        & II            & S          & M          & Linear       & Disconn & C/Disconn                    \\
		DC3-DTLZ3        & II            & S          & M          & Concave      & Disconn & C/Disconn                    \\
		DAS-CMOP1        & C             & 2          & 11         & Concave      & Disconn & C/C                    \\
		DAS-CMOP2        & C             & 2          & 11         & Mixed        & Mixed        & C/C                    \\
		DAS-CMOP3        & C             & 2          & 11         & Disconn & Disconn & C/C                    \\
		DAS-CMOP4        & C             & 2          & 11         & Concave      & Disconn & C/C                    \\
		DAS-CMOP5        & C             & 2          & 11         & Mixed        & Mixed        & C/C                    \\
		DAS-CMOP6        & C             & 2          & 11         & Disconn & Disconn & C/C                    \\
		DAS-CMOP7        & C             & 3          & 7          & Linear       & Disconn & C/C                    \\
		DAS-CMOP8        & C             & 3          & 7          & Concave      & Disconn & C/C                    \\
		DAS-CMOP9        & C             & 3          & 7          & Concave      & Disconn & C/C                    \\
		LIR-CMOP1         & IV            & 2          & 2          & Concave      & Concave      & S/Conn                       \\
		LIR-CMOP2         & IV            & 2          & 2          & Convex       & Convex       & S/Conn                       \\
		LIR-CMOP3         & IV            & 2          & 3          & Concave      & Disconn & S/Disconn                    \\
		LIR-CMOP4         & IV            & 2          & 3          & Convex       & Disconn & S/Disconn                    \\
		LIR-CMOP5         & I             & 2          & 2          & Convex       & Convex       & S/Disconn                    \\
		LIR-CMOP6         & I             & 2          & 2          & Concave      & Concave      & S/Disconn                    \\
		LIR-CMOP7         & IV            & 2          & 3          & Convex       & Concave      & S/Disconn                    \\
		LIR-CMOP8         & IV            & 2          & 3          & Concave      & Concave      & S/Disconn                    \\
		LIR-CMOP9         & II            & 2          & 2          & Concave      & Disconn & S/Disconn                    \\
		LIR-CMOP10        & II            & 2          & 2          & Convex       & Disconn & S/Disconn                    \\
		LIR-CMOP11        & III           & 2          & 2          & Convex       & Disconn & S/Disconn                    \\
		LIR-CMOP12        & III           & 2          & 2          & Concave      & Disconn & S/Disconn                    \\
		LIR-CMOP13        & I             & 3          & 2          & Mixed        & Mixed        & S/Disconn                    \\
		LIR-CMOP14        & II            & 3          & 3          & Mixed        & Mixed        & S/Disconn                    \\
		MW1              & II            & 2          & 1          & Linear       & Disconn & S/Disconn                    \\
		MW2              & I             & 2          & 1          & Linear       & Linear       & S/Disconn                    \\
		MW3              & III           & 2          & 2          & Linear       & Mixed        & S/Conn                       \\
		MW4              & I             & S          & 1          & Linear       & Linear       & S/Conn                       \\
		MW5              & II            & 2          & 3          & Concave      & Disconn & S/Conn                       \\
		MW6              & II            & 2          & 1          & Concave      & Disconn & S/Disconn                   \\
		MW7              & III           & 2          & 2          & Concave      & Disconn & S/Conn                       \\
		MW8              & II            & S          & 1          & Concave      & Disconn & S/Disconn                    \\
		MW9              & IV            & 2          & 1          & Convex       & Concave      & S/Conn                       \\
		MW10             & III           & 2          & 3          & Concave      & Disconn & S/Disconn                    \\
		MW11             & IV            & 2          & 4          & Concave      & Disconn & S/Disconn                    \\
		MW12             & IV            & 2          & 2          & Mixed        & Mixed        & S/Disconn                    \\
		MW13             & III           & 2          & 2          & Disconn & Disconn & S/Disconn                    \\
		MW14             & I             & S          & 1          & Disconn & Disconn & S/Conn                       \\ \bottomrule
	\end{tabular}
\end{table}

==> CMOP - TEVC/Tables/features.tex <==
\begin{table*}[!t]
	\centering
	\caption{The features used to characterize the Multi-Objectives Landscape of CMOP.}
	\label{tab:features3}
	\scriptsize
	\begin{tabular}{llp{9cm}lp{2cm}}
		\toprule
		Type                         & \textbf{Feature}           & \textbf{Description}                                                                                    & \textbf{Source}      & \textbf{Focus}   \\ \midrule
		\multirow{18}{*}{Global}     & upo\_n                     & Proportion of unconstrained PO solutions                                                                & \cite{Knowles2003}   & Set-Cardinality  \\
		                             & uhv                        & Hypervolume-value of the unconstrained PF                                                               & \cite{Aguirre2007}   & Set-Distribution \\
		                             & corr\_obj                  & correlation between objective values                                                                    & \cite{Liefooghe2019} & evolvability     \\
		                             & mean\_f                    & Average of unconstrained ranks                                                                          & \cite{Liefooghe2021} & y-distribution   \\
		                             & std\_f                     & Standard deviation of unconstrained ranks                                                               & \cite{Mersmann2011}  & y-distribution   \\
		                             & max\_f                     & Maximum of unconstrained ranks                                                                          & \cite{Mersmann2011}  & y-distribution   \\
		                             & skew\_f                    & Skewness of unconstrained ranks                                                                         & \cite{Mersmann2011}  & y-distribution   \\
		                             & kurt\_f                    & Kurtosis of unconstrained ranks                                                                         & \cite{Mersmann2011}  & y-distribution   \\
		                             & kurt\_avg                  & Average of objectives kurtosis                                                                          & \cite{Mersmann2011}  & y-distribution   \\
		                             & kurt\_min                  & Minimum of objectives kurtosis                                                                          & \cite{Mersmann2011}  & y-distribution   \\
		                             & kurt\_max                  & Maximum of objectives kurtosis                                                                          & \cite{Mersmann2011}  & y-distribution   \\
		                             & kurt\_rnge                 & Range of objectives kurtosis                                                                            & \cite{Mersmann2011}  & y-distribution   \\
		                             & skew\_avg                  & Average of objectives skewness                                                                          & \cite{Mersmann2011}  & y-distribution   \\
		                             & skew\_min                  & Minimum of objectives skewness                                                                          & \cite{Mersmann2011}  & y-distribution   \\
		                             & skew\_max                  & Maximum of objectives skewness                                                                          & \cite{Mersmann2011}  & y-distribution   \\
		                             & skew\_rnge                 & Range of objectives skewness                                                                            & \cite{Mersmann2011}  & y-distribution   \\
		                             & f\_mdl\_r2                 & Adjusted coefficient of determination of a linear regression model for varibles and unconstrained ranks & \cite{Mersmann2011}  & variable scaling \\
		                             & f\_range\_coeff            & Difference between maximum and minimum of the absolute value of the linear model coefficients           & \cite{Mersmann2011}  & variable scaling \\ \midrule
		\multirow{6}{*}{Random Walk} & dist\_f\_avg\_rws          & Average distance from neighbours in the objective space                                                 & \cite{Liefooghe2021} & evolvability     \\
		                             & dist\_f\_r1\_rws           & First autocorrelation coefficient of dist\_f\_avg\_rws                                                  & \cite{Liefooghe2021} & ruggedness       \\
		                             & dist\_f\_dist\_x\_avg\_rws & Ratio of dist\_f\_avg\_rws to dist\_x\_avg\_rws                                                         & \cite{Liefooghe2021} & evolvability     \\
		                             & dist\_f\_dist\_x\_avg\_r1  & First autocorrelation coefficient of dist\_f\_dist\_x\_avg\_rws                                         & \cite{Liefooghe2021} & ruggedness       \\
		                             & nuhv\_avg\_rws             & Average unconstrained hypervolume-value of neighborhood’s solutions                                     & \cite{Liefooghe2019} & evolvability     \\
		                             & nuhv\_r1\_rws              & First autocorrelation coefficient of nuhv\_avg\_rws                                                     & \cite{Liefooghe2019} & ruggedness       \\ \bottomrule
	\end{tabular}
\end{table*}

\begin{table*}[!t]
	\centering
	\caption{The features used to characterize the Violation Landscape of CMOP. The proposed features marked as New, while the (*) indicates that the feature has been modified to characterize CMOP.}
	\label{tab:features2}
	\scriptsize
	\begin{tabular}{llp{9cm}lp{2cm}}
		\toprule
		Type                          & \textbf{Feature}           & \textbf{Description}                                                                           & \textbf{Source}        & \textbf{Focus}   \\ \midrule
		\multirow{6}{*}{Global}       & min\_cv                    & Minimum of constraints violations                                                                                               & \cite{Mersmann2011} *  & y-distribution   \\
		                              & skew\_cv                   & Skewness of constraints violations                                                             & \cite{Mersmann2011} *  & y-distribution   \\
		                              & kurt\_cv                   & Kurtosis of constraints violations                                                             & \cite{Mersmann2011} *  & y-distribution   \\
		                              & cv\_mdl\_r2                & Adjusted coefficient of determination of a linear regression model for varibles and violations & \cite{Mersmann2011} *  & variable scaling \\
		                              & cv\_range\_coeff           & Difference between maximum and minimum of the absolute value of the linear model coefficients  & \cite{Mersmann2011} *  & variable scaling \\
		                              & dist\_c\_corr              & Violation-distance correlation                                                                 & \cite{Jones1995} *     & deception        \\ \midrule
		\multirow{10}{*}{Random Walk} & dist\_c\_avg\_rws          & Average distance from neighbours in the constraints space                                      & \cite{Liefooghe2021} * & evolvability     \\
		                              & dist\_c\_r1\_rws           & first autocorrelation coefficient of dist\_c\_avg\_rws                                         & \cite{Liefooghe2021} * & ruggedness       \\
		                              & dist\_c\_dist\_x\_avg\_rws & Ratio of dist\_c\_avg\_rws to dist\_x\_avg\_rws                                                & \cite{Liefooghe2021} * & evolvability     \\
		                              & dist\_c\_dist\_x\_r1\_rws  & First autocorrelation coefficient of dist\_c\_dist\_x\_avg\_rws                                & \cite{Liefooghe2021} * & ruggedness       \\
		                              & ncv\_avg\_rws              & Average single solution's violation-value                                                      & New                    & evolvability     \\
		                              & ncv\_r1\_rws               & first autocorrelation coefficient of ncv\_avg\_rws                                             & New                    & ruggedness       \\
		                              & nncv\_avg\_rws             & Average neighborhood’s violation-value                                                         & New                    & evolvability     \\
		                              & nncv\_r1\_rws              & first autocorrelation coefficient of nncv\_avg\_rws                                            & New                    & ruggedness       \\
		                              & bncv\_avg\_rws             & Average violation-value of neighborhood’s non-dominated solutions                              & New                    & evolvability     \\
		                              & bncv\_r1\_rws              & first autocorrelation coefficient of bncv\_avg\_rws                                            & New                    & ruggedness       \\ \bottomrule
	\end{tabular}
\end{table*}

\begin{table*}[!t]
	\centering
	\caption{The features used to characterize the Multi-Objectives-Violation Landscape of CMOP. The proposed features marked as New, while the (*) indicates that the feature has been modified to characterize CMOP.}
	\label{tab:features1}
	\scriptsize
	\begin{tabular}{llp{9cm}lp{2cm}}
		\toprule
		Type                          & \textbf{Feature}              & \textbf{Description}                                                        & \textbf{Source}         & \textbf{Focus}                     \\ \midrule
		\multirow{19}{*}{Global}      & fsr                           & Feasibility ratio                                                           & \cite{Malan2015}        & Set-Cardinality                    \\
		                              & po\_n                         & Proportion of PO solutions                                                  & \cite{Knowles2003}      & Set-Cardinality                    \\
		                              & hv                            & Hypervolume-value of the PF                                                 & \cite{Aguirre2007}      & Set-Distribution                   \\
		                              & cpo\_upo\_n                   & Proportion of PF to unconstrained PF                                        & New                     & PF and UPF correlation             \\
		                              & hv\_uhv\_n                    & Proportion of HV to unconstrained HV                                        & New                     & PF and UPF correlation             \\
		                              & GD\_cpo\_upo                  & distance between PF and unconstrained PF                                    & New                     & PF and UPF correlation             \\
		                              & cover\_cpo\_upo               & Proportion of unconstrained PF covered by PF                                & New                     & PF and UPF correlation             \\
		                              & corr\_cobj\_min               & Minimum constraints and objectives correlation                              & \cite{Vodopija2021}     & evolvability                       \\
		                              & corr\_cobj\_max               & Maximum constraints and objectives correlation                              & \cite{Vodopija2021}     & evolvability                       \\
		                              & corr\_cf                      & Constraints and ranks correlation                                           & \cite{Malan2015} *      & evolvability                       \\
		                              & piz\_ob\_min                  & Minimum proportion of solutions in ideal zone per objectives                & \cite{Malan2015} *      & Optima isolation                   \\
		                              & piz\_ob\_max                  & Maximum proportion of solutions in ideal zone per objectives                & \cite{Malan2015} *      & Optima isolation                   \\
		                              & piz\_f                        & Proportion of solutions in ideal zone                                       & \cite{Malan2015} *      & Optima isolation                   \\
		                              & ps\_dist\_max                 & Maximum distance across PS                                                  & \cite{Knowles2003}      & PS connectivity                    \\
		                              & ps\_dist\_mean                & Average distance across PS                                                  & \cite{Liefooghe2013b}   & PS connectivity                    \\
		                              & ps\_dist\_iqr\_mean           & Average difference between 75th and 25th percentiles of distances across PS & \cite{Liefooghe2013b}   & PS connectivity                    \\
		                              & pf\_dist\_max                 & Maximum distance across PF                                                  & \cite{Esty2022}         & PF discontinuouty                  \\
		                              & pf\_dist\_mean                & Average distance across PF                                                  & \cite{Esty2022}         & PF discontinuouty                  \\
		                              & pf\_dist\_iqr\_mean           & Average difference between 75th and 25th percentiles of distances across PF & \cite{Esty2022}         & PF discontinuouty                  \\  \midrule
		\multirow{21}{*}{Random Walk} & sup\_avg\_rws                 & Average proportion of neighbors dominating the current solution             & \cite{Liefooghe2019}    & evolvability                       \\ 
		                              & sup\_r1\_rws                  & First autocorrelation coefficient of sup\_avg\_rws                          & \cite{Liefooghe2019}    & ruggedness                         \\
		                              & inf\_avg\_rws                 & Average proportion of neighbors dominated by the current solution           & \cite{Liefooghe2019}    & evolvability                       \\
		                              & inf\_r1\_rws                  & First autocorrelation coefficient of inf\_avg\_rws                          & \cite{Liefooghe2019}    & ruggedness                         \\
		                              & inc\_avg\_rws                 & Average proportion of neighbors incomparable to the current solution        & \cite{Liefooghe2019}    & evolvability                       \\
		                              & inc\_r1\_rws                  & First autocorrelation coefficient of inc\_avg\_rws                          & \cite{Liefooghe2019}    & ruggedness                         \\
		                              & lnd\_avg\_rws                 & Average proportion of locally non-dominated solutions in the neighborhood   & \cite{Liefooghe2019}    & evolvability                       \\
		                              & lnd\_r1\_rws                  & First autocorrelation coefficient of lnd\_avg\_rws                          & \cite{Liefooghe2019}    & ruggedness                         \\
		                              & dist\_x\_avg\_rws             & Average distance from neighbours in the variable space                      & \cite{Liefooghe2021}    & evolvability                       \\
		                              & dist\_x\_r1\_rws              & First autocorrelation coefficient of dist\_x\_avg\_rws                      & \cite{Liefooghe2021}    & ruggedness                         \\
		                              & dist\_f\_c\_avg\_rws          & Average distance from neighbours in the objective-constraints space         & \cite{Liefooghe2021}  * & evolvability                       \\
		                              & dist\_f\_c\_r1\_rws           & First autocorrelation coefficient of dist\_f\_c\_avg\_rws                   & \cite{Liefooghe2021}  * & ruggedness                         \\
		                              & dist\_f\_c\_dist\_x\_avg\_rws & Ratio of dist\_f\_c\_avg\_rws to dist\_x\_avg\_rws                          & \cite{Liefooghe2021}  * & evolvability                       \\
		                              & dist\_f\_c\_dist\_x\_avg\_r1  & First autocorrelation coefficient of dist\_f\_c\_dist\_x\_avg\_rws          & \cite{Liefooghe2021}  * & ruggedness                         \\
		                              & nhv\_avg\_rws                 & Average hypervolume-value of feasible neighborhood’s solutions              & \cite{Liefooghe2019} *  & evolvability                       \\
		                              & nhv\_r1\_rws                  & First autocorrelation coefficient of nhv\_avg\_rws                          & \cite{Liefooghe2019} *  & ruggedness                         \\
		                              & bhv\_avg\_rws                 & Average hypervolume-value of neighborhood’s non-dominated solutions         & \cite{Liefooghe2019} *  & evolvability                       \\
		                              & bhv\_r1\_rws                  & First autocorrelation coefficient of bhv\_avg\_rws                          & \cite{Liefooghe2019} *  & ruggedness                         \\
		                              & nfronts\_avg\_rws             & Average number of ranks                                                     & New                     & evolvability                       \\
		                              & nfronts\_r1\_rws              & first autocorrelation coefficient of nfronts\_avg\_rws                      & New                     & ruggedness                         \\
		                              & rfbx\_rws\_avg                & Average ratio of feasible boundary crossings                                & \cite{Malan2015}        & Dispersion of the feasible regions \\ \bottomrule
	\end{tabular}
\end{table*}                 

